Graph Balancing with Orientation Costs

Motivated by the classic Generalized Assignment Problem, we consider the Graph Balancing problem in the presence of orientation costs: given an undirected multi-graph G = (V,E) equipped with edge weights and orientation costs on the edges, the goal is to find an orientation of the edges that minimizes both the maximum weight of edges oriented toward any vertex (makespan) and total orientation cost. We present a general framework for minimizing makespan in the presence of costs that allows us to: (1) achieve bicriteria approximations for the Graph Balancing problem that capture known previous results (Shmoys-Tardos [Math. Progrm. 93], Ebenlendr-Krc\'al- Sgall [Algorithmica 14], and Wang-Sitters [Inf. Process. Lett. 16]); and (2) achieve bicriteria approximations for extensions of the Graph Balancing problem that admit hyperedges and unrelated weights. Our framework is based on a remarkably simple rounding of a strengthened linear relaxation. We complement the above by presenting bicriteria lower bounds with respect to the linear programming relaxations we use that show that a loss in the total orientation cost is required if one aims for an approximation better than 2 in the makespan.

==> AdditionalIntegralityGaps.tex <==
We show an integrality gap (to LP3 or the more strong relaxation) that shows that to GB with light hyper edges, any rounding algorithm that is a $c$-approximation to the costs where $c<2$, has to be at least 1.75 approximation to the makespan.
{\color{red}This is not accurate and not interesting. It shows that if you want to get below 2 in costs then have to be at least $1.75-\epsilon$ in the makespan. But there is an integrality gap of 1.75 so not interesting. The integrality gap of 1.75 is similar to this one. just need two copies of the path and connect the $u$ vertices with each other in a light edge weight with weight $0.5$. Maybe it is interesting? because the 1.75 gap to \sGB is not valid to \LPstong with Set constraints of size 2.}
\begin{figure}[H]
	\includegraphics[width=\linewidth]{Integrality Gap3.jpeg}
	\caption{Integrality Gap3}
\end{figure}



==> Prelimilaries.tex <==
First we start with some notations regrading the \GB. Given a graph $G=(V,E)$ and a vertex $u\in V$ denote by $\delta(u)\triangleq \{e\in E\mid u\in e\}$, the collection of edges incident to $u$. In addition define: $\mathcal{F}(u)\triangleq \{S\subseteq \delta(u) \mid \sum_{e\in S} p_e \leq 1\}$, the feasible subsets of edges incident to $u$. Finally, we denote by $OPT_{LP}$ the optimal value of feasible solution to the relaxation (the exact relaxation is dependent on the context).

%Now, we present the rounding algorithm of Shmoys and Tardos to the \GAP. Given a target makespan $T$ the algorithm either outputs that there is no schedule with makespan at most $T$ or, output a schedule with makespan at most $2T$, and assignment cost of at most $C(T)$. First, the processing times are scaled by the factor $T$ so the target makespan becomes 1. 

%The algorithm is comprised of two parts: the first, solving a linear relaxation and the second, the rounding algorithm. We start by presenting the linear relaxation. Let $\mathcal{J}$ be the set of jobs and $\mathcal{M}$ be the set of machines. The linear relaxation is defined as follows:

The algorithm of Shmoys-Tardos \cite{ShmoysT93} is a key ingredient in our framework, thus we present it for completion. Recall that \cite{ShmoysT93} is a $(2,1)$-approximation for \sGAP. We assume w.l.o.g that $T=1$ (since one can scale the processing times by $T$). First, the relaxation in Figure \ref{RelaxationST} is solved, where $\mathcal{J}$ be the set of jobs and $\mathcal{M}$ be the set of machines. The variables $x_{i,j}$ for each $i\in \mathcal{M}$ and $j\in \mathcal{J}$ indicates whether job $j$ is scheduled on machine $i$. Note that if there is no feasible solution to the relaxation, then the algorithm declares there is no schedule with makespan at most $T$.

\begin{figure}
\subfloat[The relaxation by Shmoys and Trados \cite{ShmoysT93} to \sGAP.]{
		\begin{small}
			\arraycolsep=1.0pt\def\arraystretch{1.8}
			$\begin{array}{lllll}
			\text{(\LPgap)} &&&&\\
			\text{min}& \displaystyle\sum_{j\in \mathcal{J}} \sum_{i\in \mathcal{M}} x_{i,j}c_{i,j}&&&\\
			\text{s.t}& \displaystyle \sum_{i\in \mathcal{M}} x_{i,j} = 1 &&\forall j\in \mathcal{J}&(Job)\\
			& \displaystyle\sum\limits_{j\in \mathcal{J}} x_{i,j}p_{i,j} \leq 1 &&\forall i\in \mathcal{M}&(Load) \\
			& x_{i,j}=0 && \forall i\in \mathcal{M}, j\in \mathcal{J}: p_{i,j}>1&\\
			& x_{i,j} \geq 0 && \forall i\in \mathcal{M}, j\in \mathcal{J}&\\
			\end{array}$
		\end{small}

	\label{RelaxationST}
}
\subfloat[The relaxation by Ebenlendr et al. \cite{EbenlendrKS08} to \sGB.]{
		\begin{small}
			\arraycolsep=1.0pt\def\arraystretch{1.8}
			$\begin{array}{lllll}
			\text{(\LPthree)} &&&&\\
			\text{min}& \displaystyle\sum_{e\in E} \sum_{u\in e} x_{e,u}c_{e,u}&&&\\
			\text{s.t}& \displaystyle \sum_{u\in e} x_{e,u} = 1 &&\forall e\in E&(Edge)\\
			& \displaystyle\sum\limits_{e\in \delta(u)} x_{e,u}p_e \leq 1 &&\forall u\in V&(Load) \\
			& \displaystyle\sum_{e\in \delta(u):\  p_e>0.5} x_{e,u} \leq 1 &&\forall u\in V&(Star) \\
			& x_{e,u} \geq 0 && \forall u\in V, e\in \delta(u)&\\
			\end{array}$
		\end{small}
	\label{RelaxationGB}
}
\caption{The relaxation for \sGAP by \cite{ShmoysT93} and for \sGB by \cite{EbenlendrKS08}}
\label{Figure:Relaxations}
\end{figure}

Given a solution \textbf{x} to the above relaxation, the algorithm constructs a weighted bipartite graph $G=(J,S, E)$, (which will be described later). Afterwards, the algorithm finds a minimum cost perfect matching to the side $J$, i.e, each vertex in $J$ is matched to a vertex in $S$. Using this matching the algorithm assigns each job to a machine. $G$ is constructed as follows: $J=\{1,2,\ldots, n\}$ is the set of jobs, and $S$ is a set of "slots". We allocate for each machine $i$: $k_i =\lceil \sum_{j=1}^{n} x_{i,j} \rceil$ slots for jobs to be assigned to $i$. The slots for machine $i$ will be denoted by $slot(i,1),\ldots slot(i,k_i)$.

We now describe the edges $E$ (and their costs) of $G$. Each machine $i$ has $k_i$ slots with capacity 1. For each machine $i$ sort the jobs in a non-decreasing order, and for each job $j$ in that order, add $x_{i,j}$ units of job $j$ to the next non-full slot of machine $i$ (starting from $slot(i,1)$). If $x_{i,j}$ is bigger than the remaining capacity of the slot, which we denote by $r$, add $r$ units to that slot and $x_{i,j}-r$ to the next slot. %(Since $x_{i,j}\leq 1$, $x_{i,j}-r$ units will not exceed the capacity of the next slot).

We conclude the mentioned above in the following algorithm:


\begin{algorithm*}[H] \label{STrounding}
	\caption{Shmoys-Tardos $(\textbf{x}, \textbf{p})$}
	Construct the bipartite graph $G=(J,S,E)$ as described above. \\
	Find a minimum cost perfect matching with respect to $J$. \\
	For each job $j\in J$, assign $j$ to machine $i$ such that the slot $s$ that was matched to $j$, belongs to $i$.
\end{algorithm*} 

We say a slot is \textit{full} if the remaining capacity of that slot is 0. Additionally, we say a job $j$ is on top of $slot(i,s)$ if $j$ is the first job to be inserted to that slot.

It can be shown that the load on machine $i$ in the output of Algorithm \ref{STrounding} is $1+p_{i,1}$, where $p_{i,1}$ is the processing time of the job on top of $slot(i,1)$, \ie, the biggest processing time of a job that is fractionally scheduled on machine $i$. Since, $p_{i,1}\leq 1$, the makespan of the assignment is at most 2. Furthermore, it can be shown that the cost of the assignment is at most $OPT_{LP}$, and thus at most $C(T)$.

We remark that when one is aiming to solve the single criterion version of this problem, \ie, finding an assignment that minimizes the makespan, a binary search could be preformed to find the smallest $T$, such that the linear relaxation is feasible. Using Algorithm \ref{STrounding} with this target makespan gives a 2-approximation to the single criterion problem of makespan minimization.


==> Relaxation.tex <==


%The following linear relaxation is the strongest one known for the \GGB. Unfortunately, it is not known how it can be exploited to obtain better approximations for the problem.
%
%\begin{align}
%\min & \sum _{i=1}^n a_i & \label{pbjective}\\
%s.t. & x_1+x_3\leq 3 & \forall u \in V \nonumber 
%\end{align}
%
%\begin{equation}
%\begin{array}{ll@{}ll}
%\text{(CONF-LP)~~~minimize}  & \displaystyle\sum\limits_{u\in V, S\subseteq \delta(u)} x_{S,u}\sum_{e\in S} c_{e,u} &\\
%\text{subject to}
%& \displaystyle\sum\limits_{S\subseteq \delta(u)} x_{S,u} = 1 &\forall u\in V \\
%& \displaystyle\sum_{\substack{u\in V, S\subseteq \delta(u): \\ e\in S}} x_{S,u} = 1 &\forall e\in E \\
%& x_{S,u} = 0 & \forall u\in V, S\subseteq \delta(u): \sum_{e\in S} p_e > 1 \\
%& x_{S,u} \geq 0 & \forall u\in V, S\subseteq \delta(u)
%
%\end{array}
%\end{equation}

%This is believed to be the most powerful relaxation, but no rounding procedure is known to utilize the full information of this relaxation.

%In this work we use the following relaxation:

%\begin{equation*}
%\begin{array}{ll@{}ll}
%\text{(LP)~~~minimize}  & \displaystyle\sum\limits_{e=(u,v)\in E} (c_{e,u} x_{e,u} + c_{e,v} x_{e,v}) &\\
%\text{subject to}& \displaystyle x_{e,u} + x_{e,v} = 1 &\forall e=(u,v)\in E\\
%& \displaystyle\sum\limits_{e\in \delta(u)} x_{e,u}p_e \leq 1 &\forall u\in V \\
%& \displaystyle\sum_{e\in S} x_{e,u} \leq |S|-1 &\forall u\in V, S\subseteq \delta(v): \sum_{e\in S} p_e > 1 \\
%& x_{e,u} \geq 0 & \forall u\in V, e\in \delta(u)
%\end{array}
%\end{equation*}

%
%\begin{align}
%\text{(LP)}\quad\min\quad & \sum_{e=(u,v)\in E} (c_{e,u} x_{e,u} + c_{e,v} x_{e,v}) & \\
%\text{s.t.\quad} & x_{e,u} + x_{e,v} = 1 & & \forall e=(u,v)\in E & (Edge~e) \\
%& \sum\limits_{e\in \delta(u)} x_{e,u}p_e \leq 1 & & \forall u\in V & (Load~u) \\
%& \sum_{e\in S} x_{e,u} \leq |S|-1 & & \forall u\in V, S\subseteq \delta(v): S\notin \mathcal{F}(u) & (Set~u) \label{ConstraintSet}\\
%& x_{e,u} \geq 0 & & \forall u\in V, e\in \delta(u) & \nonumber
%\end{align}
%Without constraint \ref{ConstraintSet} $(LP)$ reduces to the classic relaxation given in LST which has an integrality gap of 2 with respect to the makespan.

%The next lemma shows that any feasible solution to $(CONF-LP)$ can be translated to a solution to $(LP)$.
%\begin{lemma}
%	Let $\textbf{x}$ be a feasible solution to $(CONF-LP)$ with value $M$. Then there exist a feasible solution $\textbf{y}$ to $(LP)$ with value $M$.
%\end{lemma}
%\begin{proof}
%	Let $\textbf{x}$ be a solution to $(CONF-LP)$ with value $M$. Now, define for each $e\in E$ and $u\in e$:
%	\[
%	y_{e,u} \triangleq \sum_{\substack{S\subseteq \delta(u): \\ e\in S}} x_{S,u}
%	\] 
%	
%	We will show that $\textbf{y}$ is a feasible solution to $(LP)$ with value $M$. First we'll show the value of $\textbf{y}$ in $(LP)$ is $M$:
%	\[
%	\begin{split}
%	\sum_{e=(u,v)\in E} (c_{e,u} y_{e,u} + c_{e,v} y_{e,v}) &=
%	\sum_{e=(u,v)\in E} (c_{e,u} \sum_{\substack{S\subseteq \delta(u): \\e\in S}} x_{S,u} + c_{e,v} \sum_{\substack{S\subseteq \delta(v): \\ e\in S}} x_{S,v}) \\
%	& = \sum_{u\in V, S\subseteq \delta(u)} x_{S,u}\sum_{e\in S} c_{e,u} \\
%	&= M
%	\end{split}
%	\]
%	
%	Now we'll show that $\textbf{y}$ is a feasible solution to $(LP)$. Let $e=(u,v)\in E$. Notice the Edge constraint holds since:
%	\[
%	y_{e,u} + y_{e,v} =
%	\sum_{\substack{S\subseteq \delta(u): \\ e\in S}} x_{S,u} + \sum_{\substack{S\subseteq \delta(v): \\ e\in S}} x_{S,v} =
%	\sum_{\substack{w\in V, S\subseteq \delta(w):\\ e\in S}} x_{S,w} = 1
%	\]
%	
%	In addition, given $u\in V$, The Load constraint holds since:
%	\[
%	\sum_{e\in \delta(u)} y_{e,u}p_e =
%	\sum_{e\in \delta(u)} \sum_{\substack{S\subseteq \delta(u): \\ e\in S}} x_{S,u} p_e = \sum_{S\subseteq \delta(u)} \sum_{e\in S} x_{S,u}p_e =
%	\sum_{S\subseteq \delta(u)} x_{S,u} \sum_{e\in S} p_e \leq \sum_{S\subseteq \delta(u)} x_{S,u} = 1
%	\]
%	
%	Finally, given $S\subseteq \delta(u)$ : $\sum_{e\in S} p_e > 1$, the Set constraint holds since:
%	\[
%	\sum_{e\in S} y_{e,u} =
%	\sum_{e\in S} \sum_{\substack{S\subseteq \delta(u): \\ e\in S}} x_{S,u} =
%	\sum_{T\subseteq \delta(u)} |T\cap S| \cdot x_{T,u} \overset{(1)}{\leq}
%	\sum_{T\subseteq \delta(u)} (|S|-1) \cdot x_{T,u} =
%	|S|-1
%	\]
%	(1) If $x_{T,u}>0$ then, $\sum_{e\in T} p_e\leq 1$. But since $\sum_{e\in S} p_e > 1$, then $|T\cap S|\leq |S|-1$
%\end{proof}
%
%
%To conclude, rounding our relaxation could be viewed as rounding the Configuration LP.

==> SemiRelatedULH.tex <==
In this section we discuss of a problem that captures both of the previously discussed problems of \SRGB and \GBULH. Formally, the input graph consists of edges and hyperedges. The edges, same as in the \SRGB, could have different processing times to each endpoint. Similarly, these processing times could differ by a multiplicative factor of at most $c$. In addition, the hyperedges, same as \GBULH, are unrelated but have a bounded processing time. Specifically, if $e$ is a hyperedge, and $u\in e$ then $p_{e,u}\leq \beta$. The parameters of the problem are $0\leq \beta\leq 1$, and $c\geq 1$. We call this problem \SRUH, or in short \sSRUH{$c$}{$\beta$}, where $c$ and $\beta$ are the parameters of the problem.

Note this problem captures \sGBUH{$\beta$} and \sSRGB. In this section we do something....IDK.




==> UnrelatedHeavyEdges.tex <==
%In this subsection we discuss about a new problem that naturally generalizes \sGBUH{$\beta$}. Recall the definition of a heavy edge as in the proof of Theorem \ref{Theorem:GBUH}: A heavy edge is an edge that is not a light hyperedge, and has processing time greater than $\beta$. Note that each edge is either a light hyperedge or a heavy edge.
%
%In this section we allow heavy edges to be unrelated. Formally, a heavy edge $(u,v)$ has a processing time $p_{e,u}$ or $p_{e,v}$ when orienting toward $u$ or $v$ respectively. In addition, $\beta<p_{e,u},p_{e,v}\leq 1$. However, unlike in \sGBUH{$\beta$}, $p_{e,u}$ might not equal $p_{e,v}$. We call this problem \sGBU{$\beta$}.

We start by proving that \sGBU{$\beta$} is hard as \sGAP. Formally, the following lemma gives an approximation preserving reduction from \sGAP to \sGBU{$\beta$} (the single criterion version of these problems). %This is formulated in the following lemma:

\begin{lemma} \label{HardnessLemma}
For every $0<\beta\leq 1$, if there is a $c$-approximation to \sGBU{$\beta$}, then there is a $c$-approximation to the \GAP. \footnote{We remark that by using a similar reduction, it is possible to show approximation equivalence for the bicriteria versions. Formally, if there is an $(a,b)$-approximation to \sGBU{$\beta$}, there is an $(a,b)$-approximation to \sGAP. We defer the proof for a later version of the paper.}
\end{lemma}

\begin{proof}
	For simplicity of presentation, we use the notations of jobs and machines instead of edges and vertices. Let ALG be a c-approximation to \sGBU{$\beta$}.
Given an instance of \sGAP, denote the different (sorted) values of the processing times $\textbf{p}$ by $\infty = w_0 > w_1 > w_2 > \dots > w_k$. We present in Algorithm \ref{Reduction} our approximation preserving reduction.
As previously mentioned in the paper, without loss of generality, we scale all processing times such that $max\{p_{i,j}\mid p_{i,j}\neq \infty\}=1$.
	
	\begin{algorithm*}[H] \label{Reduction}
		\caption{Reduction($\textbf{p}$)}
		\For{$\ell=1$ upto $k$}
            {If $p_{i,j} > w_\ell$, set $p_{i,j} \leftarrow \infty$.\\
			Add a new job $j'$ and two new machines $i_1$ and $i_2$ such that $p_{i_1,j'} = w_{\ell} + \epsilon$, $p_{i_2,j'} = \frac{1}{\beta}w_{\ell}$ and for every $i\notin \{i_1,i_2\}$ set $p_{i,j'} = \infty$. \\ %\footnote{In case one of the processing times is greater than 1, we scale the processing times such that $max\{p_{i,j}\mid p_{i,j}\neq \infty\}=1$} \\
			Run ALG on the new instance. %{\color{red}{WITH WHICH VALUE OF $\beta$? SHOULD IT BE $\beta = w_{\ell}$}?} \\
			Reset all changes made to $\textbf{p}$ in this iteration.
		}
		Return the best schedule among all iterations (without the job $j'$ and machines $i_1,i_2$).
	\end{algorithm*}
	
We now show that Algorithm \ref{Reduction} is a c-approximation to the given \sGAP instance.
Denote by $OPT$ the optimal makespan of the original \sGAP instance.
We note that there exists some $\ell$ such that $w_\ell \leq OPT < w_{\ell-1}$.
We prove that for this $\ell$, the $\ell$th iteration of Algorithm \ref{Reduction} produces a schedule with makespan at most $c\cdot OPT + \epsilon$ where $\epsilon > 0 $ is arbitrarily small.
	
First, note that the input is valid to ALG. This is because the only heavy job is $j'$ (the new job added in step 3), and the rest of the input (the jobs of the \sGAP instance), are light hyperedges. Thus, step 4 of Algorithm \ref{Reduction} is valid.
Second, denote by $OPT'$ the optimal makespan of the instance created in iteration $\ell$. We show that $OPT'\leq OPT + \epsilon$, which concludes the proof. A feasible orientation can orient the new added job $j'$ toward $i_1$, and the rest of the input can be oriented like in the optimal solution to the GAP instance (since $OPT<w_{\ell-1}$). The makespan of this orientation is at most $OPT'$, and thus we conclude:
	\[
	OPT' \leq max\{OPT, w_i+\epsilon\} \leq max\{OPT, OPT+\epsilon\} = OPT+\epsilon.
	\]	
\end{proof}


%{\color{red}
%We remark that the reduction for the bicriteria versions, set $p_{i,j}\leftarrow \infty$ if $p_{i,j}>T$, then adds the job $j'$ as in Algorithm \ref{Reduction}, sets $T\leftarrow T+\epsilon$ and finally executes the $(a,b)$-approximation to \sGBU{$\beta$} and returns the outputted schedule.
%}

Surprisingly, by adding a mild constraint on the value of the optimal makespan we can give an approximation better than $2$ for \sGBU{$\beta$}. The assumption is that $OPT\geq 1$, and we assume it from this point onwards. Notice that $OPT \geq 1$ holds naturally in \sGB, and \sGBUH{$\beta$}. Therefore, \sGBU{$\beta$} with the assumption that the value of the optimal makespan is at least $1$, captures these problems.
We extend our previous results to \sGBU{$\beta$} and achieve the same approximation factors for $\beta\geq \sqrt{2}-1$. To be precise, in the case that $\beta\geq \sqrt{2}-1$, we get the same result as in Theorem \ref{Theorem:GBUH}. This result is summarized in Theorem \ref{Theorem:GBU}.\footnote{We remark that makespan approximation of less than 2 is still possible with this technique for $\beta<\sqrt{2}-1$. The required threshold function can be $f(p)=1-\nicefrac{1}{x}$ for $p>\nicefrac{1}{x}$ and 1 otherwise, for sufficiently big $x$ (depends on $\beta$).}

We use Algorithm \ref{GBrounding} to prove Theorem \ref{Theorem:GBU}. Recall that given a target makespan $T$ the algorithm scales all the processing times by $T$. Similarly to \sGB, if $T<1$, the algorithm outputs that there is no orientation with makespan at most $T$. This is true since $OPT\geq 1$. Hence, similarly to \sGB we know that $p_{e,u}\leq 1$ for every $e\in E$ and $u\in e$.

The only difference in the algorithm with respect to \sGB is that if $p_{e,u}\leq 0.75+\gamma$ for every $e\in E$ and $u\in e$, we use a rounding function $f\equiv 1$. This will result a $(1.75+\gamma, 1)$-approximation as proved in \cite{ShmoysT93} (or Lemma \ref{lemmaST}). Therefore, we assume the processing times are scaled by a multiplicative factor of at least $0.75+\gamma$, \ie the target makespan $T$ satisfies $T\geq \nicefrac{1}{(0.75+\gamma)}$.


We choose the following threshold function to prove Theorem \ref{Theorem:GBU}:
\begin{align} \label{ThresholdFuncGBULHUB}
f_\alpha(p_{i,j}) =
\begin{cases}
1 & \text{if } p_{i,j}\leq \nicefrac{1}{3} \\
\alpha & \text{if } p_{i,j}> \nicefrac{1}{3} \\
\end{cases}
\end{align}
where $max\{\nicefrac{1}{3}+\nicefrac{(2\beta)}{3}, \nicefrac{2}{3}\}\leq \alpha \leq 1$.

First we upper bound the assignment cost of Algorithm \ref{GBrounding} with the above threshold function \ref{ThresholdFuncGBULHUB}.
\begin{corollary} \label{CostCorollaryGBULHUB}
	For the specific choice of a threshold function $f_\alpha$ as in \ref{ThresholdFuncGBULHUB}, the output of Algorithm \ref{GBrounding} has an assignment cost of at most $\nicefrac{1}{\alpha}\cdot C(T)$.
\end{corollary}
\begin{proof}
	The proof follows immediately from Lemma \ref{CostApprox}, which still holds for \sGBU{$\beta$}.
\end{proof}

Now we focus on bounding the makespan.
We prove that the makespan is at most $1.5 + 0.5\alpha$, and choosing $\alpha=2\gamma+0.5$ gives the desired result.

Fix a machine $i$. We use the same notations and definition as in the proof of Theorem \ref{BetterGBTheorem}. Moreover, notice that observations \ref{SetObserv}, \ref{NumOriented}, and \ref{SumRounded}, are valid in this case as well. However, note that Observation \ref{GraphObserv} does not trivially hold, even for heavy edges. This is due to the fact that the heavy edges are unrelated. We now formulate the exact observation (similar to Observation \ref{GraphObserv}) that holds for \sGBU{$\beta$}.

%and therefore after scaling the processing times, we need to guarantee that for a heavy job $j$ it holds that $f_\alpha(p_{i,j})=f_\alpha(p_{i',j})$.

\begin{observation} \label{AlmostGraphObserv}
	Let $j$ be a heavy job that isn't assigned in the \LS of Algorithm \ref{GBrounding}. Additionally, let $i$ be a machine such that $j$ could be assigned to $i$. Then, for our choice of a rounding function $f_\alpha$ it holds that $1-\alpha=1-f_\alpha(p_{i,j})\leq x_{i,j}\leq f_\alpha(p_{i,j})=\alpha$.
\end{observation}


\begin{proof}
	Let $j$ be a heavy job that isn't assigned in the \LS, and $i$ a machine such that $j$ could be assigned to $i$. The definition of a heavy job implies that before scaling the processing times (in the binary search for the optimal makespan): $p_{i,j}>\beta$.
Moreover, since we scale by a factor of at least $0.75+\gamma$, we know that after scaling the processing times satisfy $p_{i,j}>\beta(0.75+\gamma)$. Since $\gamma\geq \nicefrac{\beta}{3} -\nicefrac{1}{12}$, we can deduce:
	\begin{align*}
	p_{i,j}&>\beta(0.75+\nicefrac{1}{3}\beta -\nicefrac{1}{12})\\
	&=\beta(\nicefrac{2}{3}+\nicefrac{1}{3}\beta)\\
	&\geq 0.5(\nicefrac{2}{3}+\nicefrac{1}{3}\cdot 0.5)\\
	&\geq \nicefrac{1}{3}.
	\end{align*}
	Therefore, if $x_{i,j}>\alpha$ according to Algorithm \ref{GBrounding} and the definition of $f_\alpha$ (see \ref{ThresholdFuncGBULHUB}), $j$ should be assigned to $i$ in the \LS, which is a contradiction. Moreover, if $x_{i,j}<1-\alpha$, then $x_{i',j}>\alpha$ where $i'$ is the only machine different from $i$, that $j$ could be assigned to. Since $p_{i',j}>\nicefrac{1}{3}$ as well, $j$ should be assigned to $i'$ in the \LS, again a contradiction.
\end{proof}

Now we continue with bounding the makespan. Fix a machine $i$. We show that the load on $i$ is at most $1.5+0.5\alpha$. We use the same definitions and notations as in the previous sections. Recall that $j_1,\dots, j_k$ are the jobs on top of the slots of machine $i$, and $j'_1,j'_2$ are the jobs assigned to machine $i$ in the \LS. For simplicity of notation we use $p_\ell$ and $q_\ell$ do denote $p_{i,j_\ell}$ and $p_{i,j'_\ell}$ respectively. We consider two cases, whether $j_1$ is a heavy job or not.

\vspace{3pt}
\noindent \textbf{Case 1:} In this case $j_1$ is a heavy job. Therefore, from Lemma \ref{lemmaST} and Observation \ref{AlmostGraphObserv} the load on $i$ is at most:
\begin{align*}
&1+(1-f_\alpha(q_1))q_1+(1-f_\alpha(q_2))q_2+f_\alpha(p_1)p_1+(1-f_\alpha(p_1))p_2\\
&=1+(1-\alpha)(q_1+q_2)+\alpha p_1+(1-\alpha)p_2\\
&=1+(1-\alpha)(q_1+p_1)+(1-\alpha)(q_2+p_1)+(3\alpha-2) p_1+(1-\alpha)p_{j_2}\\
&\leq 1+(1-\alpha)+(1-\alpha)+(3\alpha-2) +(1-\alpha)\cdot 0.5\\
&=1.5+0.5\alpha.
\end{align*}
The last inequality follows from Observations \ref{SumRounded} and \ref{SecondSlotObserv}, and the fact that $(3\alpha-2)p_1$ is maximized when $p_1=1$ (this is true since $\alpha\geq \nicefrac{2}{3}$).

\vspace{3pt}
\noindent \textbf{Case 2:} In this case $j_1$ is a light job. Therefore, $p_{j_1}\leq \beta$.\footnote{Since we assume that the optimal makespan is at least 1, when scaling the processing times they do not increase.} From Lemma \ref{lemmaST}, the load on $i$ is at most:
\begin{align*}
&1+(1-f_\alpha(q_1))q_1+(1-f_\alpha(q_2))q_2+f_\alpha(p_1)p_1+(1-f_\alpha(p_1))p_2\\
&\leq 1+(1-\alpha)(q_1+q_2)+p_1\\
&\leq 1+(1-\alpha)+\beta\\
&=2-\alpha+\beta\\
&\leq 1.5+0.5\alpha.
\end{align*}
The first inequality follows from the fact that $p_2\leq p_1$. Additionally, the second inequality follows from Observation \ref{SumRounded}. Lastly, the third inequality follows from the fact that $\alpha\geq\nicefrac{1}{3}+\nicefrac{2}{3}\beta$.

From the above we can deduce the following corollary:
\begin{corollary} \label{GBUHLUBMakespanCorrol}
	The makespan of the assignment produced by Algorithm \ref{GBrounding} with a threshold function $f_\alpha$ as in \ref{ThresholdFuncGBULHUB}) is at most $1.5+0.5\alpha$.
\end{corollary}

Now we are ready to prove Theorem \ref{Theorem:GBU}.
\begin{proof}[Proof of Theorem \ref{Theorem:GBU}]
	The proof follows from Corollaries \ref{CostCorollaryGBULHUB} and \ref{GBUHLUBMakespanCorrol}, and choosing $\alpha=2\gamma+0.5$.
\end{proof}

%\noindent\inlinetitle{Integrality Gaps:}
\vspace{3pt}
\noindent {\bf Integrality Gaps:}
\input{UnrelatedHeavyIntegrality.tex}

